Instant3dit: Multiview Inpainting for Fast Editing of 3D Objects

We propose a generative technique to edit 3D shapes, represented as meshes, NeRFs, or Gaussian Splats, in approximately 3 seconds, without the need for running an SDS type of optimization. Our key insight is to cast 3D editing as a multiview image inpainting problem, as this representation is generic and can be mapped back to any 3D representation using the bank of available Large Reconstruction Models. We explore different fine-tuning strategies to obtain both multiview generation and inpainting capabilities within the same diffusion model. In particular, the design of the inpainting mask is an important factor of training an inpainting model, and we propose several masking strategies to mimic the types of edits a user would perform on a 3D shape. Our approach takes 3D generative editing from hours to seconds and produces higher-quality results compared to previous works.

==> latexmkrc.tex <==
#!/usr/bin/perl

## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.15;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";

==> tables/latex_training_strategy_table_template.tex <==

\setlength{\tabcolsep}{2pt}
\newdimen\wate \wate=30pt
\newdimen\wperc \wperc=24pt
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Prompt Adherence} & \multicolumn{3}{c}{Multi-view consistency} & \multicolumn{1}{c}{Visual quality} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-7} 
 & \multicolumn{1}{c}{ClipL$\downarrow$} & \multicolumn{1}{c}{ClipG$\uparrow$} &  \multicolumn{1}{c}{SSIM$\downarrow$} & \multicolumn{1}{c}{LPIPS$\uparrow$} & \multicolumn{1}{c}{DreamSim$\downarrow$} & \multicolumn{1}{c}{FID$\downarrow$}  \\
\midrule
\midrule
SDXL~\cite{sdxl} & aaa & aab & aac & aae & aad & aaf  \\
SDXL-inpaiting~\cite{sdxl} & caa & cab & cac & cae & cad & caf  \\
Instant3D~\cite{instant3d} & baa & bab & bac & bae & bad & baf  \\
\midrule
\ourmethod{} from Instant3D &  daa & dab & dac & dae & dad & daf  \\
\ourmethod{} from SDXL-inpainting & eaa & eab & eac & eae & ead & eaf  \\
\bottomrule
\end{tabular}


==> tables/timing_table_backbone.tex <==

\setlength{\tabcolsep}{2pt}
\newdimen\wate \wate=30pt
\newdimen\wperc \wperc=24pt
\begin{tabular}{lccccccc}
\toprule
\multirow{1}{*}{Prompt} & \multicolumn{1}{c}{p1} & \multicolumn{1}{c}{p2} & \multicolumn{1}{c}{p3} &
\multicolumn{1}{c}{p4} & \\
\midrule
\midrule
\makecell[l]{ Progressive3d \cite{cheng2024progressive3dprogressivelylocalediting}} &\cellCD[\wate]{e0a4a4}{9000}&\cellCD[\wate]{e0a4a4}{8700}&\cellCD[\wate]{e0a4a4}{13260}&\cellCD[\wate]{e0a4a4}{15000}\\
\makecell[l]{ Vox-E\cite{sella2023voxe}} &\cellCD[\wate]{e3e6bd}{2220}&\cellCD[\wate]{f6f0cb}{3000}&\cellCD[\wate]{e3e6bd}{3120}&\cellCD[\wate]{cfdcae}{2460}\\
\makecell[l]{ MVEdit \cite{mvedit2024}} &\cellCD[\wate]{bbd2a0}{744}&\cellCD[\wate]{a8c992}{528}&\cellCD[\wate]{a8c992}{663}&\cellCD[\wate]{a8c992}{462}\\ 
\makecell[l]{ NeRFiller\cite{weber2023nerfiller}} &\cellCD[\wate]{a8c992}{288}&\cellCD[\wate]{a8c992}{300}&\cellCD[\wate]{a8c992}{306}&\cellCD[\wate]{a8c992}{342}\\
\makecell[l]{ Ours} &\cellCD[\wate]{a8c992}{\textbf{3}}&\cellCD[\wate]{a8c992}{\textbf{3}}&\cellCD[\wate]{a8c992}{\textbf{3}}&\cellCD[\wate]{a8c992}{\textbf{3}}\\
\midrule

\bottomrule
\end{tabular}


==> tables/weaker_models_ablation_backbone.tex <==

% \setlength{\tabcolsep}{2pt}
% \newdimen\wate \wate=30pt
% \newdimen\wperc \wperc=24pt
% \begin{tabular}{lccccccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{Prompt Adherence} & \multicolumn{3}{c}{Multi-view consistency} & \multicolumn{1}{c}{Visual quality} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-7} 
%  & \multicolumn{1}{c}{ClipL$\downarrow$} & \multicolumn{1}{c}{ClipG$\uparrow$} &  \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} & \multicolumn{1}{c}{DreamSim$\downarrow$} & \multicolumn{1}{c}{FID$\downarrow$}  \\
% SD 1.5 &\cellCD[\wate]{f6f0cb}{27.79}&\cellCD[\wate]{feeccd}{41.33}&\cellCD[\wate]{ffe4ca}{0.72}&\cellCD[\wate]{e0a4a4}{0.09}&\cellCD[\wate]{e7b2ac}{0.6}&\cellCD[\wate]{cfdcae}{128.4} \\
% SD 2.0 &\cellCD[\wate]{e0a4a4}{27.59}&\cellCD[\wate]{e0a4a4}{40.16}&\cellCD[\wate]{e0a4a4}{0.73}&\cellCD[\wate]{e7b2ac}{0.096}&\cellCD[\wate]{e0a4a4}{0.59}&\cellCD[\wate]{cfdcae}{124.5} \\
% SDXL (ours) &\cellCD[\wate]{e3e6bd}{118.4}&\cellCD[\wate]{e3e6bd}{43.48}&\cellCD[\wate]{bbd2a0}{0.89}&\cellCD[\wate]{a8c992}{0.045}&\cellCD[\wate]{bbd2a0}{0.1}&\cellCD[\wate]{cfdcae}{118.4}\\
% \bottomrule
% \end{tabular}



\setlength{\tabcolsep}{2pt}
\newdimen\wate \wate=30pt
\newdimen\wperc \wperc=24pt
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Prompt Adherence} & \multicolumn{3}{c}{Multi-view consistency} & \multicolumn{1}{c}{Visual quality} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-7} 
 & \multicolumn{1}{c}{ClipL$\downarrow$} & \multicolumn{1}{c}{ClipG$\uparrow$} &  \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} & \multicolumn{1}{c}{DreamSim$\downarrow$} & \multicolumn{1}{c}{FID$\downarrow$}  \\
\midrule
\midrule
SD 1.5 &\cellCD[\wate]{e7b2ac}{27.79}&\cellCD[\wate]{e0a4a4}{41.33}&\cellCD[\wate]{e0a4a4}{0.719}&\cellCD[\wate]{eec0b5}{0.09}&\cellCD[\wate]{e0a4a4}{0.599}&\cellCD[\wate]{e0a4a4}{128.3} \\
SD 2.0 &\cellCD[\wate]{e0a4a4}{27.59}&\cellCD[\wate]{e0a4a4}{41.23}&\cellCD[\wate]{e0a4a4}{0.729}&\cellCD[\wate]{e0a4a4}{0.096}&\cellCD[\wate]{e7b2ac}{0.589}&\cellCD[\wate]{ffe4ca}{124.5} \\
SDXL &\cellCD[\wate]{a8c992}{\textbf{29.01}}&\cellCD[\wate]{a8c992}{\textbf{43.48}}&\cellCD[\wate]{a8c992}{\textbf{0.894}}&\cellCD[\wate]{a8c992}{\textbf{0.045}}&\cellCD[\wate]{a8c992}{\textbf{0.1}}&\cellCD[\wate]{a8c992}{\textbf{118.4}} \\
\bottomrule
\end{tabular}
